Ferrite: A Judgmental Embedding of Session Types in Rust

This paper introduces Ferrite, a shallow embedding of session types in Rust. In contrast to existing session type libraries and embeddings for mainstream languages, Ferrite not only supports linear session types but also shared session types. Shared session types allow sharing (aliasing) of channels while preserving session fidelity (preservation) using type modalities for acquiring and releasing sessions. Ferrite adopts a propositions as types approach and encodes typing derivations as Rust functions, with the proof of successful type-checking manifesting as a Rust program. We provide an evaluation of Ferrite using Servo as a practical example, and demonstrate how safe communication can be achieved in the canvas component using Ferrite.

==> sections/conclusions.tex <==
\section{Concluding Remarks}\label{sec:conclusions}

==> sections/discussion.tex <==
\section{Discussion}\label{sec:discussion}

This section reflects on our choice of host language and the guarantees provided by Ferrite and
concludes with directions for future work.

\subsection{Choice of Host Language}\label{sec:why-rust}

We chose Rust as the host language for Ferrite, as we believe in Rust's potential
for writing session type applications. Having the tagline "Fearless Concurrency"
as one of its selling points, Rust has put much effort in its language design
to ensure that concurrent programs can be written safely and efficiently.
Rust has many unique features such as ownership, borrowing, and lifetimes, amounting to an
affine type system,
which make it well suited for high performance applications.
For instance, Rust allows values to be safely modified without having to
do expensive copying, under specific conditions enforced by the type system.
Rust also provides a broad selection of high-level concurrency libraries,
such as futures, channels, async/await, which Ferrite makes use of without
having to implement the concurrency primitives from scratch.

Particularly conducive for the purpose of implementing an embedded DSL is Rust's support of functional programming
constructs, such as parametric polymorphism, traits (type classes), and
associated types (type families).   Although Rust still lacks some more advanced
language features, such as higher-kinded types and data kinds, we
managed to find alternative ways, such as using traits as indirection to
implement recursive session types in Ferrite.
Rust moreover provides excellent support for type inference, making it
possible for Ferrite programs to be written with minimal type annotations
needed.

\subsection{Guarantees}

A natural question to ask is what the guarantees are that Ferrite provides.  Since Ferrite is a
direct embedding of \SILLR, it enjoys the properties of \SILLR, assuming the absence of
implementation errors.  \SILLR in turn comprises the language $\sills$~\cite{BalzerICFP2017},
including value input and output from its precursor $\sill$~\cite{ToninhoESOP2013}, extended
with Rust statements.  Both $\sills$ and $\sill$ are proved safe, ensuring protocol adherence
in particular.  As such these guarantees directly translate into \SILLR and Ferrite, given
Ferrite's judgmental embedding of \SILLR.  This means that as long as a programmer only uses
the Ferrite library constructs made available, the session type programs are guaranteed to
comply with their defined protocol.  However, since \SILLR includes arbitrary Rust statements
and allows the input and output of arbitrary Rust values, a Ferrite session type program is
subject to all the errors that a standard Rust program can suffer from.  As a result, a Rust
\code{panic!} may be the result of executing a Ferrite session type program.

The current implementation of Ferrite simply propagates panics to the main application.  A
future improvement would be to provide explicit handling of panics raised within a
Ferrite program, so that end users are given the possibility to recover from run-time
errors. For example, one option would be to catch panics from certain Ferrite sub-programs and
convert the offered session type to an internal choice.  Alternatively, we may consider
extending Ferrite's session type language to add explicit language constructs for safe error
handling in the spirit of~\cite{FowlerPOPL2019}.

An interesting endeavor beyond the scope of this work is the proving of properties of interest
of combined Ferrite/Rust code.  For example, even though the linear fragment of $\sills$ is
proved to be deadlock-free, deadlocks may still come about from embedded Rust code.  In order to
reason about deadlock-freedom of a combined Ferrite/Rust program, the semantics of \SILLR must
be integrated with a semantics of Rust.  The RustBelt~\cite{RalfRustBelt2018} or
Oxide~\cite{AaronOxide2019} verification efforts for Rust offer valuable starting points for
such an endeavor.

\subsection{Future Work}

\paragraph{N-ary Choice}

Although not mentioned in this paper, the current implementation of Ferrite
supports \emph{binary} versions of both internal and external \emph{choice}.
There are some fine details of how Ferrite deals with the affinity constraints
for branching operations and how we work around the lack of support
for higher-rank types in Rust to encapsulate the continuation variants in
different branches.  The page limit unfortunately precludes a discussion thereof.  Currently
under development is the support of \emph{n-ary} choice, of which we have a working
prototype using \emph{row polymorphism} and \emph{prisms}.  In profunctor optics, prisms are the
duals of lenses and as such allow ``injection of a session type into a sum'' as opposed to  its
``projection from a product''.  Viewing the linear context as a product of session types and a
choice as a sum of session types, the notions of lenses and prims provide powerful abstractions
for context and choice manipulations.

\paragraph{Deep Embedding}

Ferrite currently uses the \code{async-std} library for spawning
Ferrite processes as lightweight async tasks, and uses async
channels for communication. There exist many competing concurrency
run-times for Rust other than \code{async-std},
and it may be useful if end users could choose from different run-times
when running Ferrite programs. Some users may even want to opt out
of asynchronous programming and instead use native threads for
Ferrite processes.

Unfortunately, such flexibility is not possible with Ferrit's current implementation because
Ferrite is a \textit{shallowly embedded} DSL. This means that
Ferrite programs cannot be interpreted in alternative ways, such
as using a different concurrency library or channel implementation.
We plan to explore a \textit{deep embedding} of Ferrite
to allow multiple interpretations of Ferrite programs.
Such an approach has been
explored by \cite{LindleyHaskell2016} in the context of Haskell.  A corresponding deep
embedding in Rust, however, may face challenges due to limitations of Rust's type system
mentioned in \secref{sec:why-rust}.

\paragraph{Nested Recursive Session Types}

\secref{sec:recursive-types} discusses how the type \code{Z}
is used as the type-level recursion point for a recursive session type
definition inside \code{Fix}. Generalizing this idea further,
it is possible to define \textit{nested} recursive session types
with one \code{Fix<...>} session type nested inside another
\code{Fix}. The support of such nested recursive types is possible
because we can implement \code{TypeApp} for \code{Fix} itself,
essentially lifting \code{Fix} from \code{Type} to \code{Type -> Type}.
A nested recursive session type would have multiple
recursion points, and requires the usage of \code{S<Z>} etc.
to fold and unfold from the outer \code{Fix}.
We currently have a working prototype for nested recursive
session types in Ferrite, with some details left for improving
its usability. We plan to further investigate possible use cases
 for nested recursive session types.


==> tables/old_ferrite.tex <==
\begin{table*}[t]
\caption{Overview and semantics of session types in $\sillr$ and Ferrite.}
\label{tab:sills_connectives}
\centering
\begin{footnotesize}
\renewcommand{\tabcolsep}{2mm}
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{$\sillr$} &
\textbf{Ferrite} &
\textbf{Description for Provider} \\
%
\midrule
%
$\mb{\epsilon}$ &
\texttt{End} &
Terminate session. \\
%
$\mi{\tau} \recvval A$ &
\texttt{ReceiveValue<T, A>} &
Receive value of type $\tau$, then continue as session type $A$. \\
%
$\mi{\tau} \sendval A$ &
\texttt{SendValue<T, A>} &
Send value of type $\tau$, then continue as session type $A$. \\
%
$A \chanin B$ &
\texttt{ReceiveChannel<A, B>} &
Receive channel of session type $A$, then continue as session type $B$. \\
%
$A \chanout B$ &
\texttt{SendChannel<A, B>} &
Send channel of session type $A$, then continue as session type $B$. \\
%
$A \extchoice B$ &
\texttt{ExternalChoice<Either<A, B>{}>} &
Receive label \code{Left} or \code{Right}, then continue as $A$ or $B$, respectively. \\
%
$A \intchoice B$ &
\texttt{ExternalChoice<Either<A, B>{}>} &
Send label \code{Left} or \code{Right}, then continue as $A$ or $B$, respectively. \\
%
$\extchoice\{ \overline{ l_{n}: A_{n} } \}$ &
\texttt{ExternalChoice<}$\m{HList!}[ \overline{ A_{n} } ]$\code{>} &
Receive label $l_n$, then continue as session type $A_n$. \\
%
$\intchoice\{ \overline{ l_{n}: A_{n} } \}$ &
\texttt{InternalChoice<}$\m{HList!}[\overline{ A_{n} }]$\code{>} &
Send label $l_n$, then continue as session type $A_n$. \\
%
$\lineartoshared A$ &
\texttt{LinearToShared<A>} &
Accept an acquire, then continue as a linear session type $A$. \\
%
$\sharedtolinear S$ &
\texttt{SharedToLinear<S>} &
Initiate a release, then continue as a shared session type $S$. \\
%
\bottomrule
\end{tabular}
\end{footnotesize}
\end{table*}

